An Empirical Study on Computing Equilibria in Polymatrix Games

The Nash equilibrium is an important benchmark for behaviour in systems of strategic autonomous agents. Polymatrix games are a succinct and expressive representation of multiplayer games that model pairwise interactions between players. The empirical performance of algorithms to solve these games has received little attention, despite their wide-ranging applications. In this paper we carry out a comprehensive empirical study of two prominent algorithms for computing a sample equilibrium in these games, Lemke's algorithm that computes an exact equilibrium, and a gradient descent method that computes an approximate equilibrium. Our study covers games arising from a number of interesting applications. We find that Lemke's algorithm can compute exact equilibria in relatively large games in a reasonable amount of time. If we are willing to accept (high-quality) approximate equilibria, then we can deal with much larger games using the descent method. We also report on which games are most challenging for each of the algorithms.

==> tables/auc_small/games.tex <==

\begin{tabular}{|l|c|c|c|}
\multicolumn{4}{c}{Games}\\\hline
Valuation & Auc & Types & Items\\\hline
Additive & 0 & 3 & 2\\\hline
Additive & 1 & 3 & 2\\\hline
Unit & 2 & 3 & 2\\\hline
\end{tabular}


==> tables/auc_small/lemke.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline

Time & \% Timeout \\\hline
229.442 & 13.0\\\hline
1.666 & 0.0\\\hline
427.573 & 44.5\\\hline
\end{tabular}


==> tables/auc_small/ts001.tex <==

\begin{tabular}{|c|c|c|}
\multicolumn{3}{c}{Descent 0.001}\\\hline

Time & \eps & \% Timeout \\\hline
508.037 & 5.400e-03 & 61.5\\\hline
470.797 & 3.724e-03 & 56.0\\\hline
541.041 & 2.670e-02 & 94.0\\\hline
\end{tabular}


==> tables/auc_small/ts001ls.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & \eps\\\hline
4.894 & 6.768e-04\\\hline
0.491 & 1.013e-05\\\hline
13.164 & 5.759e-03\\\hline
\end{tabular}


==> tables/auc_table/games.tex <==

\begin{tabular}{|l|c|c|c|}
\multicolumn{4}{c}{Games}\\\hline
Valuation & Auc & Types & Items\\\hline
\hhline{|=|=|=|}
Additive & FP & 3 & 3\\\hline
Additive & SP & 3 & 3\\\hline
Additive & AP & 3 & 3\\\hline
\hhline{|=|=|=|}
Unit-b2 & FP & 3 & 3\\\hline
Unit-b2 & SP & 3 & 3\\\hline
Unit-b2 & AP & 3 & 3\\\hline
\hhline{|=|=|=|}
AndOr-b2 & FP & 3 & 3\\\hline
AndOr-b2 & SP & 3 & 3\\\hline
AndOr-b2 & AP & 3 & 3\\\hline
\hhline{|=|=|=|}
Budget-b3 & FP & 3 & 3\\\hline
Budget-b3 & SP & 3 & 3\\\hline
Budget-b3 & AP & 3 & 3\\\hline
\hhline{|=|=|=|}
SingleMinded & FP & 3 & 3\\\hline
SingleMinded & SP & 3 & 3\\\hline
SingleMinded & AP & 3 & 3\\\hline
\end{tabular}


==> tables/auc_table/joint.tex <==

\begin{tabular}{|l|c|c||c|c|c||c|c||c|c|}
\multicolumn{3}{|c||}{Games} & \multicolumn{3}{c||}{\lemke} & \multicolumn{2}{c||}{\descent 0.1 LS} &
\multicolumn{2}{c|}{\descent 0.001 LS} \\\hline
Valuation & Auc & Avg. Size & Time & \% Timeout & \% Pure & Time & Eps & Time & Eps \\
\hhline{|=|=|=||=|=|=||=|=||=|=|}
Additive & FP & \multirow{3}{*}{623990} & 35.005 & 0.0 & 0.0 & 0.200 & 1.133e-02 & 1.287 & 2.630e-04\\\hline
Additive & SP &  & 0.764 & 0.0 & 100.0 & 0.233 & 7.103e-03 & 0.232 & 2.312e-05\\\hline
Additive & AP &  & 214.049 & 12.0 & 0.0 & 0.289 & 6.163e-03 & 1.610 & 1.943e-04\\
\hhline{|=|=|=||=|=|=||=|=||=|=|}
Unit-b2 & FP & \multirow{3}{*}{650417} & 46.351 & 0.0 & 34.0 & 0.199 & 6.249e-02 & 3.336 & 3.063e-02\\\hline
Unit-b2 & SP &  & 203.107 & 19.0 & 58.0 & 0.459 & 1.442e-02 & 1.831 & 2.647e-04\\\hline
Unit-b2 & AP &  & 14.709 & 0.0 & 21.0 & 0.168 & 4.182e-02 & 2.757 & 1.113e-02\\
\hhline{|=|=|=||=|=|=||=|=||=|=|}
AndOr-b2 & FP & \multirow{3}{*}{519055} & 280.322 & 23.0 & 0.0 & 0.194 & 1.927e-02 & 1.732 & 1.594e-04\\\hline
AndOr-b2 & SP &  & 1.269 & 0.0 & 100.0 & 0.279 & 7.026e-03 & 0.595 & 1.019e-04\\\hline
AndOr-b2 & AP &  & 166.011 & 9.1 & 0.0 & 0.171 & 8.662e-03 & 1.328 & 2.842e-04\\
\hhline{|=|=|=||=|=|=||=|=||=|=|}
Budget-b3 & FP & \multirow{3}{*}{647583} & 100.444 & 5.0 & 3.16 & 0.206 & 3.055e-02 & 2.003 & 4.064e-03\\\hline
Budget-b3 & SP &  & 9.438 & 1.0 & 84.85 & 0.348 & 2.543e-02 & 0.915 & 2.186e-04\\\hline
Budget-b3 & AP &  & 248.739 & 24.0 & 0.0 & 0.271 & 1.990e-02 & 2.199 & 2.233e-03\\
\hhline{|=|=|=||=|=|=||=|=||=|=|}
SingleMinded & FP & \multirow{3}{*}{606511} & 82.166 & 7.37 & 5.0 & 0.139 & 2.775e-02 & 1.551 & 1.822e-03\\\hline
SingleMinded & SP &  & 110.341 & 17.0 & 48.19 & 0.475 & 1.045e-02 & 1.359 & 1.669e-04\\\hline
SingleMinded & AP &  & 59.942 & 3.0 & 1.0 & 0.162 & 1.856e-02 & 1.544 & 1.038e-03\\\hline\end{tabular}


==> tables/auc_table/lemke.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline

Time & \% Timeout \\\hline
\hhline{|=|=|}
35.005 & 0.0\\\hline
0.764 & 0.0\\\hline
214.049 & 12.0\\\hline
\hhline{|=|=|}
46.351 & 0.0\\\hline
203.107 & 19.0\\\hline
14.709 & 0.0\\\hline
\hhline{|=|=|}
280.322 & 23.0\\\hline
1.269 & 0.0\\\hline
166.011 & 9.1\\\hline
\hhline{|=|=|}
100.444 & 5.0\\\hline
9.438 & 1.0\\\hline
248.739 & 24.0\\\hline
\hhline{|=|=|}
82.166 & 5.0\\\hline
110.341 & 17.0\\\hline
59.942 & 3.0\\\hline
\end{tabular}


==> tables/auc_table/ts001.tex <==

\begin{tabular}{c|c|c|c}
\multicolumn{4}{c}{Descent LS 0.1}\\\hline

Time & Iterations & Eps & \% Timeout \\\hline


==> tables/auc_table/ts001ls.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Eps &\\\hline
\hhline{|=|=|}
1.287 & 2.630e-04\\\hline
0.232 & 2.312e-05\\\hline
1.610 & 1.943e-04\\\hline
\hhline{|=|=|}
3.336 & 3.063e-02\\\hline
1.831 & 2.647e-04\\\hline
2.757 & 1.113e-02\\\hline
\hhline{|=|=|}
1.732 & 1.594e-04\\\hline
0.595 & 1.019e-04\\\hline
1.328 & 2.842e-04\\\hline
\hhline{|=|=|}
2.003 & 4.064e-03\\\hline
0.915 & 2.186e-04\\\hline
2.199 & 2.233e-03\\\hline
\hhline{|=|=|}
1.551 & 1.822e-03\\\hline
1.359 & 1.669e-04\\\hline
1.544 & 1.038e-03\\\hline
\end{tabular}


==> tables/auc_table/ts1ls.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.1}\\\hline

Time & Eps &\\\hline
\hhline{|=|=|}
0.200 & 1.133e-02\\\hline
0.233 & 7.103e-03\\\hline
0.289 & 6.163e-03\\\hline
\hhline{|=|=|}
0.199 & 6.249e-02\\\hline
0.459 & 1.442e-02\\\hline
0.168 & 4.182e-02\\\hline
\hhline{|=|=|}
0.194 & 1.927e-02\\\hline
0.279 & 7.026e-03\\\hline
0.171 & 8.662e-03\\\hline
\hhline{|=|=|}
0.206 & 3.055e-02\\\hline
0.348 & 2.543e-02\\\hline
0.271 & 1.990e-02\\\hline
\hhline{|=|=|}
0.139 & 2.775e-02\\\hline
0.475 & 1.045e-02\\\hline
0.162 & 1.856e-02\\\hline
\end{tabular}


==> tables/blotto/games.tex <==

\begin{tabular}{|l|c|c|c|}
\multicolumn{4}{c}{Games}\\\hline
Game & Hills & Types & Troops\\\hline
AdjWinner & 3 & 3 & 8\\\hline
AdjWinner & 3 & 3 & 10\\\hline
AdjWinner & 3 & 3 & 12\\\hline
AdjWinner & 3 & 4 & 8\\\hline
AdjWinner & 3 & 4 & 9\\\hline
AdjWinner & 3 & 4 & 10\\\hline
BlottoPayoff & 3 & 3 & 8\\\hline
BlottoPayoff & 3 & 3 & 10\\\hline
BlottoPayoff & 3 & 3 & 12\\\hline
BlottoPayoff & 4 & 3 & 4\\\hline
BlottoPayoff & 4 & 3 & 5\\\hline
BlottoPayoff & 4 & 3 & 6\\\hline
\end{tabular}


==> tables/blotto/lemke.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline

Time & \% Timeout \\\hline
0.248 & 0.0\\\hline
0.493 & 0.0\\\hline
12.725 & 2.0\\\hline
0.527 & 0.0\\\hline
0.726 & 0.0\\\hline
0.870 & 0.0\\\hline
71.814 & 0.0\\\hline
382.497 & 23.0\\\hline
573.663 & 91.0\\\hline
12.114 & 0.0\\\hline
87.155 & 0.0\\\hline
499.651 & 49.0\\\hline
\end{tabular}


==> tables/blotto/ts001ls.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Avg Eps \\\hline
0.188 & 1.654e-03\\\hline
0.342 & 2.002e-03\\\hline
0.569 & 1.864e-03\\\hline
0.344 & 2.273e-03\\\hline
0.456 & 2.155e-03\\\hline
0.604 & 2.254e-03\\\hline
0.477 & 5.281e-04\\\hline
0.843 & 5.408e-04\\\hline
1.405 & 6.268e-04\\\hline
0.292 & 4.980e-04\\\hline
0.583 & 4.913e-04\\\hline
1.106 & 5.088e-04\\\hline
\end{tabular}


==> tables/blotto/ts1.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.1}\\\hline

Time & Avg Eps \\\hline
0.028 & 2.237e-02\\\hline
0.048 & 2.229e-02\\\hline
0.079 & 2.558e-02\\\hline
0.047 & 2.474e-02\\\hline
0.063 & 2.693e-02\\\hline
0.084 & 2.752e-02\\\hline
0.059 & 1.417e-02\\\hline
0.151 & 1.684e-02\\\hline
0.263 & 1.547e-02\\\hline
0.018 & 9.091e-03\\\hline
0.036 & 7.473e-03\\\hline
0.075 & 5.867e-03\\\hline
\end{tabular}


==> tables/coord_joint.tex <==

\begin{tabular}{|c|c||c|c||c|c||c|c|}
\multicolumn{2}{|c||}{Games} & \multicolumn{2}{c||}{\lemke} & \multicolumn{2}{c||}{\descent 0.1 LS} &
\multicolumn{2}{c|}{\descent 0.001 LS} \\\hline
Graph & $p$ & Time & \% Timeout & Time & Eps & Time & Eps \\
\hhline{|=|=||=|=||=|=||=|=|}
Complete & 0 & 1.270 & 0.0 & 0.034 & 2.103e-02 & 0.760 & 9.951e-04\\\hline
Complete & 0.25 & 63.407 & 4.0 & 0.033 & 2.115e-02 & 0.748 & 1.026e-03\\\hline
Complete & 0.5 & 337.443 & 45.0 & 0.034 & 1.859e-02 & 0.750 & 1.070e-03\\\hline
Complete & 0.75 & 522.207 & 74.0 & 0.033 & 1.604e-02 & 0.725 & 1.076e-03\\\hline
Complete & 1 & 116.354 & 0.0 & 0.034 & 4.844e-03 & 0.598 & 5.087e-04\\\hhline{|=|=||=|=||=|=||=|=|}
Cycle & 0 & 18.430 & 2.0 & 0.103 & 3.352e-02 & 3.612 & 1.093e-03\\\hline
Cycle & 0.25 & 184.451 & 21.0 & 0.103 & 3.157e-02 & 3.534 & 1.167e-03\\\hline
Cycle & 0.5 & 412.947 & 55.0 & 0.105 & 2.859e-02 & 3.430 & 1.136e-03\\\hline
Cycle & 0.75 & 593.414 & 96.0 & 0.103 & 2.626e-02 & 3.206 & 1.121e-03\\\hline
Cycle & 1 & 600.097 & 100.0 & 0.107 & 1.906e-02 & 2.712 & 6.557e-04\\\hhline{|=|=||=|=||=|=||=|=|}
Grid & 0 & 35.447 & 3.0 & 0.072 & 3.143e-02 & 2.257 & 1.023e-03\\\hline
Grid & 0.25 & 260.455 & 35.0 & 0.069 & 3.239e-02 & 2.233 & 1.137e-03\\\hline
Grid & 0.5 & 451.699 & 61.0 & 0.072 & 2.955e-02 & 2.254 & 1.170e-03\\\hline
Grid & 0.75 & 552.286 & 82.0 & 0.072 & 2.786e-02 & 2.106 & 1.186e-03\\\hline
Grid & 1 & 599.349 & 99.0 & 0.070 & 2.159e-02 & 1.802 & 6.489e-04\\\hhline{|=|=||=|=||=|=||=|=|}
Tree & 0 & 0.276 & 0.0 & 0.060 & 1.012e-02 & 0.818 & 1.175e-03\\\hline
Tree & 0.25 & 0.542 & 0.0 & 0.062 & 1.997e-02 & 0.806 & 1.220e-03\\\hline
Tree & 0.5 & 73.443 & 5.0 & 0.062 & 2.139e-02 & 0.814 & 1.246e-03\\\hline
Tree & 0.75 & 165.418 & 4.0 & 0.061 & 2.150e-02 & 0.796 & 1.084e-03\\\hline
Tree & 1 & 162.420 & 0.0 & 0.063 & 1.469e-03 & 0.778 & 7.686e-04\\\hline\end{tabular}


==> tables/games_coord.tex <==

\begin{tabular}{|l|c|c|}
\multicolumn{2}{c}{Games}\\\hline
Graph & p \\\hline
Complete & 0\\\hline
Complete & 0.25\\\hline
Complete & 0.5\\\hline
Complete & 0.75\\\hline
Complete & 1\\\hhline{|=|=|}
Cycle & 0\\\hline
Cycle & 0.25\\\hline
Cycle & 0.5\\\hline
Cycle & 0.75\\\hline
Cycle & 1\\\hhline{|=|=|}
Grid & 0\\\hline
Grid & 0.25\\\hline
Grid & 0.5\\\hline
Grid & 0.75\\\hline
Grid & 1\\\hhline{|=|=|}
Tree & 0\\\hline
Tree & 0.25\\\hline
Tree & 0.5\\\hline
Tree & 0.75\\\hline
Tree & 1\\\hline
\end{tabular}


==> tables/games_gzero.tex <==

\begin{tabular}{|l|c|c|}
\multicolumn{2}{c}{Games}\\\hline
\# Payoff& p \\\hline
20250.0 & 2\\\hline
20250.0 & 3\\\hline
20250.0 & 5\\\hhline{|=|=|}
26010.0 & 2\\\hline
26010.0 & 3\\\hline
26010.0 & 5\\\hhline{|=|=|}
36000.0 & 2\\\hline
36000.0 & 3\\\hline
36000.0 & 5\\\hline
\end{tabular}


==> tables/games_strict.tex <==

\begin{tabular}{|l|c|c|}
\multicolumn{2}{c}{Games}\\\hline
Graph & p \\\hline
Complete & 5\\\hhline{|=|=|}
Cycle & 5\\\hhline{|=|=|}
Grid & 5\\\hhline{|=|=|}
Tree & 5\\\hline
\end{tabular}


==> tables/games_weight.tex <==

\begin{tabular}{|l|c|c|}
\multicolumn{2}{c}{Games}\\\hline
Graph & p \\\hline
Complete & 2\\\hline
Complete & 5\\\hhline{|=|=|}
Cycle & 2\\\hline
Cycle & 5\\\hhline{|=|=|}
Grid & 2\\\hline
Grid & 5\\\hhline{|=|=|}
Tree & 2\\\hline
Tree & 5\\\hline
\end{tabular}


==> tables/gzero_joint.tex <==

\begin{tabular}{|c|c||c|c||c|c||c|c|}
\multicolumn{2}{|c||}{Games} & \multicolumn{2}{c||}{\lemke} & \multicolumn{2}{c||}{\descent 0.1 LS} &
\multicolumn{2}{c|}{\descent 0.001 LS} \\\hline
Graph & $p$ & Time & \% Timeout & Time & Eps & Time & Eps \\
\hhline{|=|=||=|=||=|=||=|=|}
\multirow{3}{*}{20250} & 2 & 368.032 & 36.0 & 0.025 & 1.976e-02 & 0.577 & 1.093e-03\\\cline{2-8}
 & 3 & 495.919 & 66.0 & 0.026 & 1.762e-02 & 0.571 & 1.131e-03\\\cline{2-8}
 & 5 & 435.207 & 29.0 & 0.025 & 1.308e-02 & 0.531 & 9.926e-04\\\hhline{|=|=||=|=||=|=||=|=|}
\multirow{3}{*}{26010.0} & 2 & 438.650 & 59.0 & 0.035 & 1.855e-02 & 0.775 & 1.068e-03\\\cline{2-8}
 & 3 & 576.439 & 91.0 & 0.035 & 1.583e-02 & 0.756 & 1.120e-03\\\cline{2-8}
 & 5 & 582.924 & 88.0 & 0.034 & 1.186e-02 & 0.686 & 9.738e-04\\\hhline{|=|=||=|=||=|=||=|=|}
\multirow{3}{*}{36000.0} & 2 & 545.997 & 84.0 & 0.053 & 1.564e-02 & 1.092 & 1.049e-03\\\cline{2-8}
& 3 & 598.616 & 99.0 & 0.053 & 1.396e-02 & 1.074 & 1.110e-03\\\cline{2-8}
& 5 & 600.088 & 100.0 & 0.052 & 1.101e-02 & 0.982 & 9.721e-04\\\hline\end{tabular}


==> tables/lemke_coord.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline
Time & \% Timeout \\\hline
1.270 & 0.0\\\hline
63.407 & 4.0\\\hline
337.443 & 45.0\\\hline
522.207 & 74.0\\\hline
116.354 & 0.0\\\hhline{|=|=|}
18.430 & 2.0\\\hline
184.451 & 21.0\\\hline
412.947 & 55.0\\\hline
593.414 & 96.0\\\hline
600.097 & 100.0\\\hhline{|=|=|}
35.447 & 3.0\\\hline
260.455 & 35.0\\\hline
451.699 & 61.0\\\hline
552.286 & 82.0\\\hline
599.349 & 99.0\\\hhline{|=|=|}
0.276 & 0.0\\\hline
0.542 & 0.0\\\hline
73.443 & 5.0\\\hline
165.418 & 4.0\\\hline
162.420 & 0.0\\\hline
\end{tabular}


==> tables/lemke_gzero.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline
Time & \% Timeout \\\hline
368.032 & 36.0\\\hline
495.919 & 66.0\\\hline
435.207 & 29.0\\\hhline{|=|=|}
438.650 & 59.0\\\hline
576.439 & 91.0\\\hline
582.924 & 88.0\\\hhline{|=|=|}
545.997 & 84.0\\\hline
598.616 & 99.0\\\hline
600.088 & 100.0\\\hline
\end{tabular}


==> tables/lemke_strict.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline
Time & \% Timeout \\\hline
356.009 & 17.0\\\hhline{|=|=|}
580.891 & 85.0\\\hhline{|=|=|}
551.795 & 77.0\\\hhline{|=|=|}
79.560 & 0.0\\\hhline{|=|=|}
\end{tabular}


==> tables/lemke_weight.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Lemke}\\\hline
Time & \% Timeout \\\hline
0.113 & 0.0\\\hline
0.050 & 0.0\\\hhline{|=|=|}
0.168 & 0.0\\\hline
0.129 & 0.0\\\hhline{|=|=|}
0.122 & 0.0\\\hline
0.089 & 0.0\\\hhline{|=|=|}
0.177 & 0.0\\\hline
0.144 & 0.0\\\hline
\end{tabular}


==> tables/multi/games.tex <==

\begin{tabular}{|l|c|c|}
\multicolumn{3}{c}{Games}\\\hline
Valuation & Auc & Avg. Size\\\hline
Additive & D & \multirow{3}{*}{836465}\\\hline
Additive & U & \\\hline
Additive & AP & \\\hline
SubModular & D & \multirow{3}{*}{878491}\\\hline
SubModular & U & \\\hline
SubModular & AP & \\\hline
\end{tabular}


==> tables/multi/joint.tex <==

\begin{tabular}{|l|c|c|c||c|c||c|c||c|c|}
\multicolumn{4}{|c||}{Games} & \multicolumn{2}{c||}{\lemke} & \multicolumn{2}{c||}{\descent 0.1 LS} &
\multicolumn{2}{c|}{\descent 0.001 LS} \\\hline
Valuation & Auc & Avg. Size & Time & \% Timeout & Time & Eps & Time & Eps \\
\hhline{|=|=|=||=|=||=|=||=|=|}
Additive & D & 3 & 3 & 9.504 & 0.0 & 30.0 & 0.295 & 1.452e-02 & 1.481 & 4.411e-04\\\hline
Additive & U & 3 & 3 & 0.954 & 0.0 & 100.0 & 0.380 & 1.321e-02 & 1.870 & 3.579e-04\\\hline
Additive & AP & 3 & 3 & 512.564 & 64.0 & 0.0 &  0.417 & 4.080e-03 & 2.182 & 3.170e-04\\\hhline{|=|=|=||=|=||=|=||=|=|}
SubModular & D & 3 & 3 & 29.054 & 0.0 & 5.0 & 0.270 & 1.326e-02 & 1.954 & 3.209e-04\\\hline
SubModular & U & 3 & 3 & 5.818 & 0.0 & 83.0 & 0.272 & 2.636e-02 & 1.741 & 8.645e-04\\\hline
SubModular & AP & 3 & 3 & 210.290 & 12.0 & 0.0 & 0.323 & 1.115e-02 & 2.192 & 3.273e-04\\\hline\end{tabular}


==> tables/multi/lemke.tex <==

\begin{tabular}{|c|c|c|}
\multicolumn{3}{c}{Lemke}\\\hline

Time & \% Timeout & \% Pure \\\hline
6.255 & 0.0 & 67.0 \\\hline
0.958 & 0.0 & 100.0 \\\hline
473.103 & 53.0 & 0.0 \\\hline
21.172 & 0.0 & 18.0 \\\hline
6.402 & 0.0 & 89.0 \\\hline
220.444 & 18.0 & 0.0 \\\hline
\end{tabular}


==> tables/multi/ts001.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent 0.001}\\\hline

Time & Iterations & Eps & \% Timeout \\\hline
0.519 & 2.0 & 1.396e-02 & 0.0\\\hline
0.565 & 1.3 & 1.578e-02 & 0.0\\\hline
0.600 & 1.4 & 5.963e-03 & 0.0\\\hline
0.391 & 2.0 & 1.350e-02 & 0.0\\\hline
0.407 & 1.3 & 2.462e-02 & 0.0\\\hline
0.451 & 2.0 & 1.129e-02 & 0.0\\\hline
\end{tabular}


==> tables/multi/ts001ls.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Eps \\\hline
1.338 & 1.513e-03\\\hline
1.486 & 4.055e-04\\\hline
1.589 & 2.328e-04\\\hline
1.442 & 6.161e-04\\\hline
1.483 & 8.924e-04\\\hline
1.677 & 2.536e-04\\\hline
\end{tabular}


==> tables/multi/ts1ls.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent 0.1}\\\hline

Time & Eps \\\hline
0.319 & 1.807e-02\\\hline
0.345 & 1.700e-02\\\hline
0.468 & 3.456e-03\\\hline
0.272 & 1.442e-02\\\hline
0.282 & 2.471e-02\\\hline
0.321 & 1.094e-02\\\hline
\end{tabular}


==> tables/strict_joint.tex <==

\begin{tabular}{|c|c||c|c||c|c||c|c|}
\multicolumn{2}{|c||}{Games} & \multicolumn{2}{c||}{\lemke} & \multicolumn{2}{c||}{\descent 0.1 LS} &
\multicolumn{2}{c|}{\descent 0.001 LS} \\\hline
Graph & $p$ & Time & \% Timeout & Time & Eps & Time & Eps \\
\hhline{|=|=||=|=||=|=||=|=|}
Complete & 5 & 356.009 & 17.0 & 0.024 & 1.878e-02 & 0.552 & 1.054e-03\\\hhline{|=|=||=|=||=|=||=|=|}
Cycle & 5 & 580.891 & 85.0 & 0.087 & 1.729e-02 & 2.102 & 1.068e-03\\\hhline{|=|=||=|=||=|=||=|=|}
Grid & 5 & 551.795 & 77.0 & 0.066 & 1.612e-02 & 1.428 & 1.108e-03\\\hhline{|=|=||=|=||=|=||=|=|}
Tree & 5 & 79.560 & 0.0 & 0.048 & 2.571e-03 & 0.664 & 8.111e-04\\\hline\end{tabular}


==> tables/ts001ls_coord.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Avg Eps\\\hline
0.762 & 9.951e-04\\
\hline
0.760 & 1.026e-03\\
\hline
0.765 & 1.070e-03\\
\hline
0.737 & 1.076e-03\\
\hline
0.604 & 5.087e-04\\
\hhline{|=|=|}
3.660 & 1.093e-03\\
\hline
3.581 & 1.167e-03\\
\hline
3.478 & 1.136e-03\\
\hline
3.243 & 1.121e-03\\
\hline
2.739 & 6.557e-04\\
\hhline{|=|=|}
2.284 & 1.023e-03\\
\hline
2.270 & 1.137e-03\\
\hline
2.293 & 1.170e-03\\
\hline
2.138 & 1.186e-03\\
\hline
1.811 & 6.489e-04\\
\hhline{|=|=|}
0.807 & 1.175e-03\\
\hline
0.804 & 1.220e-03\\
\hline
0.822 & 1.246e-03\\
\hline
0.804 & 1.084e-03\\
\hline
0.781 & 7.686e-04\\
\hline
\end{tabular}


==> tables/ts001ls_gzero.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Avg Eps\\\hline
0.577 & 1.093e-03\\
\hline
0.571 & 1.131e-03\\
\hline
0.531 & 9.926e-04\\
\hhline{|=|=|}
0.775 & 1.068e-03\\
\hline
0.756 & 1.120e-03\\
\hline
0.686 & 9.738e-04\\
\hhline{|=|=|}
1.092 & 1.049e-03\\
\hline
1.074 & 1.110e-03\\
\hline
0.982 & 9.721e-04\\
\hline
\end{tabular}


==> tables/ts001ls_strict.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Avg Eps\\\hline
0.565 & 1.054e-03\\
\hhline{|=|=|}
2.121 & 1.068e-03\\
\hhline{|=|=|}
1.444 & 1.108e-03\\
\hhline{|=|=|}
0.673 & 8.111e-04\\
\hhline{|=|=|}
\end{tabular}


==> tables/ts001ls_weight.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.001}\\\hline

Time & Avg Eps\\\hline
0.593 & 7.370e-04\\
\hline
0.863 & 7.156e-04\\
\hhline{|=|=|}
4.190 & 7.782e-04\\
\hline
3.463 & 6.098e-04\\
\hhline{|=|=|}
2.458 & 6.149e-04\\
\hline
2.056 & 7.221e-04\\
\hhline{|=|=|}
1.568 & 7.612e-04\\
\hline
0.977 & 7.646e-04\\
\hline
\end{tabular}


==> tables/ts1ls_coord.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.1}\\\hline

Time & Avg Eps\\\hline
0.033 & 2.103e-02\\
\hline
0.034 & 2.115e-02\\
\hline
0.034 & 1.859e-02\\
\hline
0.034 & 1.604e-02\\
\hline
0.035 & 4.844e-03\\
\hhline{|=|=|}
0.104 & 3.352e-02\\
\hline
0.104 & 3.157e-02\\
\hline
0.106 & 2.859e-02\\
\hline
0.104 & 2.626e-02\\
\hline
0.108 & 1.906e-02\\
\hhline{|=|=|}
0.073 & 3.143e-02\\
\hline
0.070 & 3.239e-02\\
\hline
0.073 & 2.955e-02\\
\hline
0.073 & 2.786e-02\\
\hline
0.070 & 2.159e-02\\
\hhline{|=|=|}
0.060 & 1.012e-02\\
\hline
0.062 & 1.997e-02\\
\hline
0.062 & 2.139e-02\\
\hline
0.061 & 2.150e-02\\
\hline
0.063 & 1.469e-03\\
\hline
\end{tabular}


==> tables/ts1ls_gzero.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.1}\\\hline

Time & Avg Eps\\\hline
0.025 & 1.976e-02\\
\hline
0.026 & 1.762e-02\\
\hline
0.025 & 1.308e-02\\
\hhline{|=|=|}
0.035 & 1.855e-02\\
\hline
0.035 & 1.583e-02\\
\hline
0.034 & 1.186e-02\\
\hhline{|=|=|}
0.053 & 1.564e-02\\
\hline
0.053 & 1.396e-02\\
\hline
0.052 & 1.101e-02\\
\hline
\end{tabular}


==> tables/ts1ls_strict.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.1}\\\hline

Time & Avg Eps\\\hline
0.024 & 1.878e-02\\
\hhline{|=|=|}
0.088 & 1.729e-02\\
\hhline{|=|=|}
0.066 & 1.612e-02\\
\hhline{|=|=|}
0.047 & 2.571e-03\\
\hhline{|=|=|}
\end{tabular}


==> tables/ts1ls_weight.tex <==

\begin{tabular}{|c|c|}
\multicolumn{2}{c}{Descent LS 0.1}\\\hline

Time & Avg Eps\\\hline
0.017 & 5.522e-03\\
\hline
0.013 & 6.601e-03\\
\hhline{|=|=|}
0.022 & 5.625e-03\\
\hline
0.015 & 4.546e-03\\
\hhline{|=|=|}
0.020 & 4.753e-03\\
\hline
0.013 & 4.620e-03\\
\hhline{|=|=|}
0.020 & 2.821e-04\\
\hline
0.016 & 7.897e-03\\
\hline
\end{tabular}


==> tables/weight_joint.tex <==

\begin{tabular}{|c|c||c|c||c|c||c|c|c|}
\multicolumn{2}{|c||}{Games} & \multicolumn{2}{c||}{\lemke} & \multicolumn{2}{c||}{\descent 0.1 LS} &
\multicolumn{3}{c|}{\descent 0.001 LS} \\\hline
Graph & $p$ & Time & \% Timeout & Time & Eps & Time & Eps & \% Timeout \\
\hhline{|=|=||=|=||=|=||=|=|=|}
Complete & 2 & 194.233 & 8.0 & 8.455 & 1.446e-02 & 86.116 & 9.603e-04 & 0.0 \\\hline
Complete & 3 & 410.118 & 38.0 & 6.551 & 1.909e-02 & 73.485 & 1.047e-03 & 0.0 \\\hline
Complete & 5 & 552.583 & 81.0 & 4.957 & 2.585e-02 & 64.676 & 1.130e-03 & 0.0
\\\hhline{|=|=||=|=||=|=||=|=|=|}
Cycle & 2 & 103.403 & 0.0 & 0.227 & 1.334e-01 & 577.984 & 3.094e-02 & 73.0 \\\hline
Cycle & 3 & 90.062 & 0.0 & 0.172 & 1.412e-01 & 529.581 & 4.199e-02 & 48.0 \\\hline
Cycle & 5 & 78.883 & 0.0 & 0.156 & 1.427e-01 & 438.707 & 3.950e-02 & 28.0
\\\hhline{|=|=||=|=||=|=||=|=|=|}
Grid & 2 & 116.157 & 0.0 & 0.864 & 8.298e-02 & 275.839 & 5.461e-03 & 1.0 \\\hline
Grid & 3 & 81.933 & 0.0 & 0.464 & 1.110e-01 & 480.608 & 1.368e-02 & 15.0 \\\hline
Grid & 5 & 58.054 & 0.0 & 0.131 & 1.384e-01 & 358.662 & 3.028e-02 & 2.0
\\\hhline{|=|=||=|=||=|=||=|=|=|}
Tree & 2 & 240.215 & 0.0 & 0.750 & 0.000e+00 & 2.768 & 3.253e-04 & 0.0\\\hline
Tree & 3 & 220.510 & 0.0 & 0.709 & 0.000e+00 & 2.533 & 1.194e-04 & 0.0\\\hline
Tree & 5 & 204.919 & 0.0 & 0.653 & 0.000e+00 & 2.345 & 8.947e-05 & 0.0\\\hline\end{tabular}

